Recitation-Augmented Language Models

We propose a new paradigm to help Large Language Models (LLMs) generate more accurate factual knowledge without retrieving from an external corpus, called RECITation-augmented gEneration (RECITE). Different from retrieval-augmented language models that retrieve relevant documents before generating the outputs, given an input, RECITE first recites one or several relevant passages from LLMs' own memory via sampling, and then produces the final answers. We show that RECITE is a powerful paradigm for knowledge-intensive NLP tasks. Specifically, we show that by utilizing recitation as the intermediate step, a recite-and-answer scheme can achieve new state-of-the-art performance in various closed-book question answering (CBQA) tasks. In experiments, we verify the effectiveness of \method~on four pre-trained models (PaLM, UL2, OPT, and Codex) and three CBQA tasks (Natural Questions, TriviaQA, and HotpotQA). Our code is available at "https://github.com/Edward-Sun/RECITE".

==> feedback.tex <==
LGTM. This paper proposed a recite-and-answer algorithm that achieves new state-of-the-art few-shot results on the closed-book question answering (CBQA) task. The approach is interesting and explores new capabilities of Large Language Models (LLM) prompting.

No concerns are found related to confidential or proprietary information. The paper uses PaLM, UL2, and OPT that are publicly known to external audiences. The datasets used (Natural Questions, TriviaQA, HotpotQA) are all public.

Some detailed feedback are as follows.

Abstraction/Introduction, it’s good to explicitly state by how much that this work improves over the SOTA benchmark results.

Sec 3, para 2. I don’t understand this sentence “top-retrieved Wikipedia pages for queries issued to the Google search engine by multiple users”. What are the queries and who are the users? How many queries are needed? If a lot are needed, then it becomes less preferable. Apparently this is related to the fine-tuning section, and please refer to my later feedback regarding that.

Sec 3.1 Figure 2 in sub-figure 2), it shows that the LM input is “<Recitation N> <Question 0> <Answer 0> … <Question N>”. Would it be more accurate to be “<Question 0> <Recitation 0> <Answer 0> … <Question N> <Recitation N>”?

Sec 3.1 para 1. I don’t understand what this sentence is about: “finding the evidence passage after generating the answer”.

Sec 3.2. It seems to me that generating sub-questions is a non-trivial new task. Hence the actual prompts for that should be discussed in the main text or appendix. Currently it is omitted (Figure 3). Its effectiveness should also be discussed for the same reason.

Sec 3.2 Figure 3 shows that Q1, Q2, and Q3 are sort of in parallel. But actually the generation of Q2 depends on the result of Q1, and Q3 depends on Q1 and Q2. Figure 3 may be revised to reflect the sequential dependency between sub-questions.

Sec 3.3. I didn’t fully understand the motivation of “fine-tuning on few-shot generated questions” or how it is done. In addition, discussing the fine-tuning topic makes the paper’s main theme (which I think focuses on few-shot prompting) less clear. Consider to remove it if not critically necessary.

Sec 3.3. I see that the term “diversified recitation” is being used to refer to “passage hint-based diversified recitation” in the later experimental section. However, the basic version discussed in section 3.1 already includes “sampling top-k recitations” before doing self-consistency, which can also be viewed as generating “diversified” recitations already (controlled by temperature). I suggest using the full term “passage hint-based diversified recitation” across the paper to reduce confusion.

Sec 4.2. Is the baseline (Standard-prompting) from existing reference work or self-implemented? Does it represent SOTA?

Sec 4.2.1 Why not report “recite-and-answer w/ diversified recitation results” for TQ?

Sec 4.3. More experimental analysis and ablation studies could be helpful. For example, (1) evaluate the accuracy of the recitation passage (Is it identical to some desirable reference passage? is it relevant? Is it factually correct? ). (2) Comparing the accuracy of the recite module with some retrieval methods (BM25 or REALM etc.). (3) Headroom analysis, for example, if we manually do the recite work and feed the model with the ideal recitation passages, what would the final accuracy be like? (4) Error analysis, e.g., how many examples are incorrect due to errors in sub-questions generation, recitation error, or final answer generation, or self-consistency?
